Learning Open Domain Multi-hop Search Using Reinforcement Learning

We propose a method to teach an automated agent to learn how to search for multi-hop paths of relations between entities in an open domain. The method learns a policy for directing existing information retrieval and machine reading resources to focus on relevant regions of a corpus. The approach formulates the learning problem as a Markov decision process with a state representation that encodes the dynamics of the search process and a reward structure that minimizes the number of documents that must be processed while still finding multi-hop paths. We implement the method in an actor-critic reinforcement learning algorithm and evaluate it on a dataset of search problems derived from a subset of English Wikipedia. The algorithm finds a family of policies that succeeds in extracting the desired information while processing fewer documents compared to several baseline heuristic algorithms.

==> content/dataset.tex <==
To evaluated the focused reading learning method, we introduce a novel dataset derived from the English version of Wikipedia.
Our dataset consist of a set of 369 multi-hop search problems, where
a search problem is consists of a pair of entities to be connected by a path of relations, potentially connecting to other entities along the path. 
% if the correct documents in the corpus are retrieved and processed with an information extraction component. % ms: redundant

The foundation of the dataset is a subset of 6,880 Wikipedia articles from the WikiHop~\cite{welbl-etal-2018-constructing} corpus. We used Wikification~\cite{RRDA11, cheng-roth-2013-relational} to extract named entities from these documents and normalize them to the title of a corresponding Wikipedia article. 
%We ran Wikification ahead of time over 6,880 wikipedia articles.
%
Wikification does not perform relation extraction, so we lack gold-standard relations. To overcome this limitation, in this paper we induce a relation between entities that co-occur within a window of three sentences. Every relation extracted this way can be traced back to at least one document in the corpus.

We create a gold-standard knowledge graph using the induced entities and relations, and we sample pairs of entities connected by paths to create search problems for the dataset. Table \ref{tab:dataset} contains a break-down of the number of elements in each subset of the dataset. Figure \ref{fig:hops} shows the distribution of path lengths (number of hops) between target entities in the test problems. To avoid overlap between training and test data, none of the target endpoints are shared between the train and test data.


%The information retrieval component is an inverted index built on top of the same subset of documents, 
We train an LDA model\footnote{We used the LDA implementation provided by gensim \url{https://radimrehurek.com/gensim_3.8.3/}.} and constructed an information retrieval inverted index over the collection of documents.\footnote{The dataset files, with the documents, extractions, indices and LDA model will be made public upon acceptance of the article.}


%\todo{If you have space, you should include a histogram for the length of the paths in these queries. It would be nice to understand how multi-hop it really is.}


